Invisible Watermarks, Visible Gains: Steering Machine Unlearning with Bi-Level Watermarking Design

With the increasing demand for the right to be forgotten, machine unlearning (MU) has emerged as a vital tool for enhancing trust and regulatory compliance by enabling the removal of sensitive data influences from machine learning (ML) models. However, most MU algorithms primarily rely on in-training methods to adjust model weights, with limited exploration of the benefits that data-level adjustments could bring to the unlearning process. To address this gap, we propose a novel approach that leverages digital watermarking to facilitate MU by strategically modifying data content. By integrating watermarking, we establish a controlled unlearning mechanism that enables precise removal of specified data while maintaining model utility for unrelated tasks. We first examine the impact of watermarked data on MU, finding that MU effectively generalizes to watermarked data. Building on this, we introduce an unlearning-friendly watermarking framework, termed Water4MU, to enhance unlearning effectiveness. The core of Water4MU is a bi-level optimization (BLO) framework: at the upper level, the watermarking network is optimized to minimize unlearning difficulty, while at the lower level, the model itself is trained independently of watermarking. Experimental results demonstrate that Water4MU is effective in MU across both image classification and image generation tasks. Notably, it outperforms existing methods in challenging MU scenarios, known as "challenging forgets".

==> sec/sec_MU_for_watermark_v0.tex <==
\SL{[Remove the following.]}

\begin{tcolorbox}[colframe=blue!80!black, colback=blue!10!white, coltitle=black, sharp corners, boxrule=0.8mm, width=\linewidth]
\textbf{Summary of insights into watermarked data in MU}
\\[1ex]
Watermarked data does \textit{not} have a significant impact on the general unlearning process. MU can generalize to watermarked data for `free'.
\end{tcolorbox}

In this section, we analyze the impact of watermarking on MU. Specifically, we aim to investigate how would a watermarked forget/retain set with random secret information possibly influence the performance of MU? The watermarked data can be introduced either during the \textit{unlearning} phase or the \textit{evaluation} phase. So we can summarize four possible scenarios: a) clean data for unlearning and clean data for evaluation, b) clean data for unlearning and watermarked data for evaluation, c) watermarked data for unlearning and clean data for evaluation and d) watermarked data for unlearning and watermarked data for evaluation, as shown in \cref{tab:scen}.

\begin{table}[htpb]
\centering
\caption{Summary of integrating watermarking into MU scenarios.}
\begin{tabular}{|c|c|c|}
\hline
Scenario & Data in unlearning & Data in evaluation     \\ \hline
$\mathcal U_1$& $\mathcal D$ & $\mathcal D$            \\ \hline
$\mathcal U_2$& $\mathcal D$ & $\hat{\mathcal D}$      \\ \hline
$\mathcal U_3$& $\hat{\mathcal D}$ & $\mathcal D$      \\ \hline
$\mathcal U_4$& $\hat{\mathcal D}$ & $\hat{\mathcal D}$\\ \hline
\end{tabular}
\label{tab:scen}
\end{table}
Our preliminary study cover two commonly used MU methods, fine-tuning (FT) and gradient ascent (GA). FT fine-tunes the trained model $\btheta_\mathrm{o}$ on $\mathcal D_\mathrm{r}$ to initiate the forgetting over $\mathcal D_\mathrm{f}$. GA reverses the model training using gradient ascent on $\mathcal D_\mathrm{f}$ with the same training loss as pre-training. From the above, we can see that FT relies solely on $\mathcal D_\mathrm{r}$ while GA uses only $\mathcal D_\mathrm{f}$. 

We use a pre-trained {\hidden} network $f_{\btheta_\mathrm{w}}$ to encode random message $\mathbf m$ into forget set $\mathcal D_\mathrm{f}$ and retain set $\mathcal D_\mathrm{r}$. Then, we apply MU on the obtained watermarked forget set $\hat{\mathcal D_\mathrm{f}}$ and retain set $\hat{\mathcal D_\mathrm{r}}$: 
\begin{align}
    \btheta_\mathrm{u}^{\mathrm{w}}=\argmin_\btheta \lambda_\mathrm{f}\ell_\mathrm{f}(\btheta;\hat{\mathcal D_\mathrm{f}})+\lambda_\mathrm{r}\mathcal \ell_\mathrm{r}(\btheta;\hat{\mathcal D_\mathrm{r}}),
\label{eq:3}
\end{align}
where $\lambda_\mathrm{f}=0$ for FT and $\lambda_\mathrm{r}=0$ for GA. Specifically, during this MU process, we conduct 10\% random data forgetting on the pre-trained \textsc{ResNet-18} network on \textsc{CIFAR-10} dataset. Next, we compare the unlearning effectiveness and retaining performance of the corresponding unlearned model $\btheta_u$ with and without watermarking. Specifically, we look into unlearning accuracy (UA), defined as $1-\text{Acc}_{\mathcal D_\mathrm{f}}(\btheta_\mathrm{u})$, and membership inference attack (MIA), which indicates how likely the samples in $\mathcal D_\mathrm{f}$ are predicted as forgetting samples. The model utility of $\btheta_\mathrm{u}$ is also assessed with the metrics including retaining accuracy (RA), define as the accuracy of $\btheta_\mathrm{u}$ on $\mathcal D_\mathrm{r}$, and test accuracy (TA), the accuracy of $\btheta_\mathrm{u}$ on the test set. The results are shown in \cref{tab:scen_ft,tab:scen_ga}. 
\begin{table}[t]
\caption{Performance of FT unlearning under random forgetting at different scenarios on \textsc{CIFAR-10}.}
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Scenarios      & Unlearned model                 & UA   & MIA  & RA    & TA    \\ \hline
Retrain & -           & 6.78 & 16.06 & 100.00 & 92.02 \\ \hline
$\mathcal U_1$ & $\btheta_\mathrm{u}$            & 1.85 & 5.60 & 99.66 & 93.54 \\ \hline
$\mathcal U_2$ & $\btheta_\mathrm{u}$            & 4.78 & 0.33 & 96.27 & 90.22 \\ \hline
$\mathcal U_3$ & $\btheta_\mathrm{u}^\mathrm{w}$ & 1.36 & 4.08 & 99.85 & 93.65 \\ \hline
$\mathcal U_4$ & $\btheta_\mathrm{u}^\mathrm{w}$ & 3.23 & 1.97 & 98.90 & 91.83 \\ \hline
\end{tabular}
}
\label{tab:scen_ft}
\end{table}

\begin{table}[t]
\caption{Performance of GA unlearning under random forgetting at different scenarios on \textsc{CIFAR-10}.}
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Scenarios      & Unlearned model                 & UA   & MIA  & RA    & TA    \\ \hline
Retrain & -           & 6.78 & 16.06 & 100.00 & 92.02 \\ \hline
$\mathcal U_1$ & $\btheta_\mathrm{u}$            & 0.80 & 1.89 & 99.42 & 94.19 \\ \hline
$\mathcal U_2$ & $\btheta_\mathrm{u}$            & 5.25 & 0.82 & 94.92 & 89.01 \\ \hline
$\mathcal U_3$ & $\btheta_\mathrm{u}^\mathrm{w}$ & 0.73 & 1.87 & 99.38 & 93.66 \\ \hline
$\mathcal U_4$ & $\btheta_\mathrm{u}^\mathrm{w}$ & 5.37 & 1.27 & 95.39 & 89.41 \\ \hline
\end{tabular}
}
\label{tab:scen_ga}
\end{table}
\begin{table}[t]
\caption{Performance of FT unlearning under class forgetting at different scenarios on \textsc{CIFAR-10}.}
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Scenarios      & Unlearned model                 & UA    & MIA   & RA    & TA    \\ \hline
$\mathcal U_1$ & $\btheta_\mathrm{u}$            & 12.51 & 20.98 & 99.73 & 92.04 \\ \hline
$\mathcal U_2$ & $\btheta_\mathrm{u}$            & 32.43 & 22.97 & 91.68 & 82.84 \\ \hline
$\mathcal U_3$ & $\btheta_\mathrm{u}^\mathrm{w}$ & 10.06 & 16.60 & 99.74 & 92.94 \\ \hline
$\mathcal U_4$ & $\btheta_\mathrm{u}^\mathrm{w}$ & 26.14 & 16.60 & 93.82 & 86.82 \\ \hline
\end{tabular}
}
\end{table}
As we can see, using watermarked data for unlearning does \textit{not} have a significant impact on the general unlearning performance and no significant improvement or drop can be observed. This indicates that MU can generalize to watermarked data for `free'. However, it still remains elusive what secret information in the watermark can positively influence the unlearning performance? Further, we wonder if watermarks can be specifically designed or optimized to enhance unlearning performance. In the next section, we will answer these questions by connecting the watermark for MU with bi-level optimization problem.
